Fully Latent Principal Stratification With Measurement Models

There is wide agreement on the importance of implementation data from randomized effectiveness studies in behavioral science; however, there are few methods available to incorporate these data into causal models, especially when they are multivariate or longitudinal, and interest is in low-dimensional summaries. We introduce a framework for studying how treatment effects vary between subjects who implement an intervention differently, combining principal stratification with latent variable measurement models; since principal strata are latent in both treatment arms, we call it "fully-latent principal stratification" or FLPS. We describe FLPS models including item-response-theory measurement, show that they are feasible in a simulation study, and illustrate them in an analysis of hint usage from a randomized study of computerized mathematics tutors.

==> cutText.tex <==
Assumption \eqref{eq:independenceX} states that conditional on $\etat$, implementation indicators $\bm{M}$ are independent of covariates $\bm{x}$. 
This assumption is not quite as strong as it may seem since $\etat$ itself is modeled as a function of covariates. 
For instance, we will consider models of $\bm{M}$ based on the Rasch structure 
where $logit^{-1}(x)=(1+e^{-x})^{-1}$ is the inverse logit function, $d_j$ is a ``difficulty'' parameter that varies by item but not by student, and $\etati\sim \mathcal{N}(\bm{x}_i\bm{\beta},\sigma^2)$ for coefficients $\bm{\beta}$ and variance $\sigma^2$. This is equivalent to a standard multilevel logistic regression where $Pr(M_{ij}=1)=logit^{-1}(\beta_0+\bm{x}_i'\bm{\beta}+\xi_i-d_j)$ with a student random intercept $\xi$. % and a linear component, that varies with $i$. 
Then, \eqref{eq:independenceX} is equivalent to the assumption that the logistic regression fits well, i.e. fully captures the relationship between $\bm{x}$ and $\bm{M}$. 
In fact, assumption \eqref{eq:independenceX} could be weakened, or done away with entirely


%The data revolution in education has led to more data collection within randomized controlled trials (RCTs) to study program effectiveness. It is particularly the case in RCTs involving computer-based interventions, which allow researchers and administrators to collect implementation data in the form of log or clickstream data. For example, \citeA{pane2014effectiveness} conducted a large-scale RCT to study the effectiveness of using computers in math learning. This study gathered not only primary data for evaluating program effectiveness, but also collected log data from intelligent tutoring that include students’ performance on each worked section, timestamps, and hints requested. Such log data present an unprecedented opportunity for researchers in understanding how and why online interventions work.

%Despite the potential of RCT with computer-based interventions, log data pose a challenge since it differs in structure and size from the type of data commonly observed in studies of causal mechanisms. Unlike the implementation or mediation data that most current statistical techniques are designed for, computer log data are highly multivariate, multilevel, and messy. Taking \citeauthor{pane2014effectiveness}'s study as an example, their data were gathered from 147 schools, spanning 52 diverse school districts in seven states over the course of two school years. In addition, the log data (e.g., mastery data) were available only for students assigned to the treatment group who could have access to the software for intervention. Furthermore, some log data, including the number of problems, widely varied among students in the treatment group \cite{aoas}. As a result, traditional statistical methods developed for causal models do not adapt easily to computer-intervened RCT data.

%To exploit complex log data structure, fully-latent Principal Stratification (FLPS) was proposed, incorporating a latent-variable-based measurement component into a broader causal model. The technique is an extension of principal stratification \cite[PS;][]{frangakis2002principal}, a causal framework used for studying how treatment effects vary as a function of post-treatment or intermediate variables \cite{aoas}. Such FLPS modeling opens the door in causal modeling---combining PS and other causal frameworks with measurement models, such as item response theory. The proposed method can incorporate continuous latent variables into PS via measurement models, substantially extending the scope of PS modeling to multivariate and complex implementation data.

% The FLPS framework could significantly influence RCT analysis, particularly when big implementation data are available, such as in evaluations of computer-based interventions. 
%The purpose of this study is to evaluate performance of the FLPS framework in incorporating various item response models. We consider a two-parameter logistic (2PL) model, a generalized partial credit model, and a graded response model to describe ordinal response measurement data and investigate performance of FLPS in conducting causal inference. The paper is structured as follows. The following section provides a brief description of the statistical underpinnings of PS and FLPS. % In the next section, we explicate how PS can be extended to FLPS with latent measurement models incorporated. 
%The following sections present a simulation study that evaluates the performance of FLPS. The FLPS is then applied to empirical data to show an example application. The paper concludes with a discussion of the findings and future directions.

As an alternative, “Fully Latent PS” or “FLPS” extends classic PS to model implementation data, including several measurements of an underlying construct of interest, say $\boldsymbol{M}_{i}$ for subjects $i$ assigned to the treatment condition.
In this manuscript, we will focus on the common scenario in education in which each measurement recorded in $\bm{M}$ corresponded to a specific item $j=1,\dots,J$. 
For instance, in \citeA{aoas}, the items were units from the curriculum of an educational computer application, so $M_{ij}$ recorded whether student $i$ mastered the material in unit $j$, and in the example in Section \ref{sec:realData}, the items are practice problems and $M_{ij}$ measures the amount of feedback student $i$ received while working on practice problem $j$. 
In these examples, most students do not have measurements for every item---for instance, most students did not work on every available practice problem.
When no measurement is available for student $i$ on item $j$, we will write $\bM_{ij}=\NA$. 




%The data revolution in education has led to more data collection within randomized controlled trials (RCTs) to study program effectiveness. It is particularly the case in RCTs involving computer-based interventions, which allow researchers and administrators to collect implementation data in the form of log or clickstream data. For example, \citeA{pane2014effectiveness} conducted a large-scale RCT to study the effectiveness of using computers in math learning. This study gathered not only primary data for evaluating program effectiveness, but also collected log data from intelligent tutoring that include students’ performance on each worked section, timestamps, and hints requested. Such log data present an unprecedented opportunity for researchers in understanding how and why online interventions work.

%Despite the potential of RCT with computer-based interventions, log data pose a challenge since it differs in structure and size from the type of data commonly observed in studies of causal mechanisms. Unlike the implementation or mediation data that most current statistical techniques are designed for, computer log data are highly multivariate, multilevel, and messy. Taking \citeauthor{pane2014effectiveness}'s study as an example, their data were gathered from 147 schools, spanning 52 diverse school districts in seven states over the course of two school years. In addition, the log data (e.g., mastery data) were available only for students assigned to the treatment group who could have access to the software for intervention. Furthermore, some log data, including the number of problems, widely varied among students in the treatment group \cite{aoas}. As a result, traditional statistical methods developed for causal models do not adapt easily to computer-intervened RCT data.

%To exploit complex log data structure, fully-latent Principal Stratification (FLPS) was proposed, incorporating a latent-variable-based measurement component into a broader causal model. The technique is an extension of principal stratification \cite[PS;][]{frangakis2002principal}, a causal framework used for studying how treatment effects vary as a function of post-treatment or intermediate variables \cite{aoas}. Such FLPS modeling opens the door in causal modeling---combining PS and other causal frameworks with measurement models, such as item response theory. The proposed method can incorporate continuous latent variables into PS via measurement models, substantially extending the scope of PS modeling to multivariate and complex implementation data.

% The FLPS framework could significantly influence RCT analysis, particularly when big implementation data are available, such as in evaluations of computer-based interventions. 
%The purpose of this study is to evaluate performance of the FLPS framework in incorporating various item response models. We consider a two-parameter logistic (2PL) model, a generalized partial credit model, and a graded response model to describe ordinal response measurement data and investigate performance of FLPS in conducting causal inference. The paper is structured as follows. The following section provides a brief description of the statistical underpinnings of PS and FLPS. % In the next section, we explicate how PS can be extended to FLPS with latent measurement models incorporated. 
%The following sections present a simulation study that evaluates the performance of FLPS. The FLPS is then applied to empirical data to show an example application. The paper concludes with a discussion of the findings and future directions.














To overcome this situation, Bayesian estimation is applied to the proposed model. Let $\boldsymbol{\theta}$% = (\tau_0, \tau_1, \omega, \boldsymbol{\beta}, \boldsymbol{\gamma}, \boldsymbol{a}, \boldsymbol{d})$ 
contain the free parameters of FLPS. %, where $\tau_0$ and $\tau_1$ model the principal effects (i.e., intercept, slope), $\omega$ model the effect of the latent factor, and $\boldsymbol{\beta}$ and $\boldsymbol{\gamma}$ each model the covariate effects on $\eta$ and $Y$. 
%$\boldsymbol{a}$ and $\boldsymbol{b}$ each model the slopes and intercepts of the measurement variables. 
For estimation, one specifies four sub-models:

- $f(Y_C|\boldsymbol{x}, \eta_T; \boldsymbol{\theta})$: a model for control potential outcomes as a function of covariates $\boldsymbol{x}$ and latent parameters $\eta_T$

- $f(Y_T|\boldsymbol{x}, \eta_T; \boldsymbol{\theta})$: an analogous model for treatment potential outcomes

- $f(\boldsymbol{m_i}| \eta_T; \boldsymbol{\theta})$: a measurement model

- $f(\eta_T| \boldsymbol{x}; \boldsymbol{\theta})$: a model for $\eta_T$ as a function of $\boldsymbol{x}$


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> outcomeRegSmall.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Mon Jun  5 19:38:16 2023
\begin{tabular}{llll}
  \hline
  & Rasch & 2PL & GRM \\ 
   \hline
$\omega$ & 0.463 *** & 0.354 *** & 0.324 *** \\ 
   & (0.063) & (0.045) & (0.047) \\ 
  $\tau_0$ & --0.011 & 0.016 & 0.03 \\ 
   & (0.036) & (0.038) & (0.038) \\ 
  $\tau_1$ & 0.033 & 0.062 & 0.043 \\ 
   & (0.036) & (0.036) & (0.036) \\ 
   \hline
$R^2$ & 0.526 & 0.619 & 0.634 \\ 
   \hline
\multicolumn{4}{l}{  *** p < 0.001;  ** p < 0.01;  * p < 0.05. }  
  \end{tabular}


==> table1.tex <==

\begin{tabular}[t]{llll}
\toprule
  & Delayed & Immediate & Overall\\
\midrule
 & (N=388) & (N=416) & (N=804)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Pretest}}\\
\hspace{1em} &  &  \vphantom{10} & \\
\hspace{1em}Mean (SD) & 4.76 (2.67) & 4.91 (2.64) & 4.84 (2.65)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{5th Grd State Test}}\\
\hspace{1em} &  &  \vphantom{9} & \\
\hspace{1em}Mean (SD) & 581 (58.8) & 580 (59.1) & 581 (58.9)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Sex}}\\
\hspace{1em}Female & 176 (45.4\%) & 204 (49.0\%) & 380 (47.3\%)\\
\hspace{1em}Male & 212 (54.6\%) & 212 (51.0\%) & 424 (52.7\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Race/Ethnicity}}\\
\hspace{1em}White & 186 (47.9\%) & 226 (54.3\%) & 412 (51.2\%)\\
\hspace{1em}Hispanic/Latino & 57 (14.7\%) & 51 (12.3\%) & 108 (13.4\%)\\
\hspace{1em}Asian & 109 (28.1\%) & 109 (26.2\%) & 218 (27.1\%)\\
\hspace{1em}Other & 36 (9.3\%) & 30 (7.2\%) & 66 (8.2\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Accelerated}}\\
\hspace{1em} & 95 (24.5\%) & 94 (22.6\%) & 189 (23.5\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{EIP}}\\
\hspace{1em} & 28 (7.2\%) & 29 (7.0\%) & 57 (7.1\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Gifted}}\\
\hspace{1em} & 75 (19.3\%) & 75 (18.0\%) & 150 (18.7\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{IEP}}\\
\hspace{1em} & 37 (9.5\%) & 41 (9.9\%) & 78 (9.7\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{ESOL}}\\
\hspace{1em} & 38 (9.8\%) & 34 (8.2\%) & 72 (9.0\%)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Days Absent (6th Grd)}}\\
\hspace{1em} &  &  \vphantom{8} & \\
\hspace{1em}Median [IQR] & 2.46 [3.87] & 2.58 [3.74] & 2.52 [3.83]\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Avg. Time on Tasks (Pretest)}}\\
\hspace{1em} &  &  \vphantom{7} & \\
\hspace{1em}Median [IQR] & 1.04 [0.895] & 1.06 [0.880] & 1.05 [0.903]\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Math Anxiety}}\\
\hspace{1em} &  &  \vphantom{6} & \\
\hspace{1em}Mean (SD) & 13.5 (5.64) & 13.5 (5.74) & 13.5 (5.69)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Math Self-Efficacy}}\\
\hspace{1em} &  &  \vphantom{5} & \\
\hspace{1em}Mean (SD) & 17.5 (4.81) & 17.7 (4.72) & 17.6 (4.76)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Perceptual Sensitivity}}\\
\hspace{1em} &  &  \vphantom{4} & \\
\hspace{1em}Mean (SD) & 7.67 (2.91) & 7.66 (2.92) & 7.66 (2.91)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{\% Correct w/o Feedback}}\\
\hspace{1em} &  &  \vphantom{3} & \\
\hspace{1em}Mean (SD) & NA & 65.9 (16.1) & 65.9 (16.1)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{\% Partial Feedback}}\\
\hspace{1em} &  &  \vphantom{2} & \\
\hspace{1em}Mean (SD) & NA & 23.2 (7.93) & 23.2 (7.93)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{\% Bottom Out}}\\
\hspace{1em} &  &  \vphantom{1} & \\
\hspace{1em}Mean (SD) & NA & 10.9 (12.2) & 10.9 (12.2)\\
\addlinespace[0.3em]
\multicolumn{4}{l}{\textbf{Posttest}}\\
\hspace{1em} &  &  & \\
\hspace{1em}Mean (SD) & 9.04 (1.01) & 9.05 (0.994) & 9.05 (0.999)\\
\bottomrule
\end{tabular}


==> to_do.tex <==

- edit everything
% - online appendix
- Take out classic ps from applied section
- Put reference to data source in data section 
- concluding remark on real data analysis
    - Discuss differences between model results
    - models are robust

- data: plural vs singular consistent

% - bibtex references

% - paragraph indents?


